ReasonXL: A Large-Scale Corpus for Language-Specific Reasoning in LLMs

Despite advances in multilingual capabilities, most large language models (LLMs) remain English-centric in their training and, crucially, in the reasoning traces they produce: even for non-English problems, they predominantly reason in English, leaving non-English users with intermediate reasoning they cannot follow. We address this disparity with two contributions. **(a)** We introduce $\texttt{ReasonXL}$, the first large-scale parallel corpus of cross-domain reasoning traces in five European languages (English, German, French, Italian, and Spanish): over 2.5M aligned samples (11B tokens) per language, each comprising prompt, reasoning trace, and final output, enabling direct supervision of language-specific reasoning. **(b)** Using $\texttt{ReasonXL}$, we demonstrate that LLMs can be adapted to reason entirely in a target language through a simple two-stage pipeline of supervised fine-tuning (SFT) and reinforcement learning with verifiable rewards (RLVR), matching or exceeding the base models' English-reasoning performance in two of four languages and recovering most of it in the remaining two.

==> sections/05_evaluation.tex <==
\section{A Representational Analysis on the Effects of Reasoning Tuning}
\label{sec:mech}

To understand \emph{how} language-specific reasoning adaptation reshapes the model internals, we conduct a mechanistic analysis comparing the base \texttt{SmolLM3}, SFT, and final RL checkpoints. 
All analyses in this section are performed on 250 French MGSM prompts; results for the other languages follow similar patterns and are in Appendix \ref{app:mech_interp}.

\subsection{Weight Change Analysis}

We measure the relative Frobenius-norm change $\|\Delta W\|_F / \|W_{\text{ref}}\|_F$ for every weight matrix in the network \citep{lee2019wide}, grouping tensors by layer and module type (attention projections and MLP projections). 
For each layer we report the mean and standard deviation across component tensors within that layer. 

Figure~\ref{fig:mechanistic-weights} shows the resulting layer-wise profiles. 
Both attention and MLP modules exhibit a clear depth-dependent pattern: weight updates grow monotonically with layer index, concentrating the largest changes in the upper third of the network. 
SFT and RL produce nearly overlapping curves when measured against the base model, indicating that the bulk of the parameter shift is established during the SFT stage. 
In contrast, the additional RL update over SFT (green, right axis) is an order of magnitude smaller and distributed more uniformly across depth. 
This suggests that RL acts as a targeted refinement step rather than a second large-scale reparameterization.

\begin{figure}[t]
    \centering

    % Top legends
    \begin{subfigure}[t]{0.65\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/legend_pairs.pdf}
    \end{subfigure}
    
    % ---- Row 1 ----
    \begin{minipage}{0.45\linewidth}
        \centering
        \begin{subfigure}[t]{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{assets/summary_attn.pdf}
            \caption{Attention} %  Weight Change
        \end{subfigure}
    \end{minipage}
    \hspace{0.02\linewidth}
    \begin{minipage}{0.45\linewidth}
        \centering
        \begin{subfigure}[t]{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{assets/summary_mlp.pdf}
            \caption{MLP} %  Weight Change
        \end{subfigure}
    \end{minipage}
        
    \caption{
    Analysis of weight changes across training stages (Base $\to$ SFT $\to$ RL) for \underline{French}.
    \textbf{(a,b)} Relative weight change per layer shows a clear depth-dependent pattern for both attention and MLP modules: updates are consistently larger in the later (upper) layers of the model. \textbf{SFT and RL both induce substantial shifts from the Base model in these deeper layers, whereas the additional RL updates over SFT are markedly smaller in magnitude and more evenly distributed across depth.} % The results for the other languages follow similar patterns and are provided in the Appendix.
    }

    \label{fig:mechanistic-weights}
\end{figure}

\begin{figure}[t]
    \centering

    % Top legend
    \begin{subfigure}[t]{0.65\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/legend_pairs.pdf}
    \end{subfigure}

    \begin{minipage}{0.45\linewidth}
        \centering
        \begin{subfigure}[t]{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{assets/cosine_sim_last_token.pdf}
            \caption{Activation Drift}
        \end{subfigure}
    \end{minipage}
    \hspace{0.01\linewidth}
    \begin{minipage}{0.45\linewidth}
        \centering
        \begin{subfigure}[t]{\linewidth}
            \centering
            \includegraphics[width=\linewidth]{assets/patching_language_shift.pdf}
            \caption{Activation Patching}
        \end{subfigure}
    \end{minipage}
    % \hspace{0.01\linewidth}
    % \begin{minipage}{0.30\linewidth}
    %     \centering
    %     \begin{subfigure}[t]{\linewidth}
    %         \centering
    %         \resizebox{\linewidth}{!}{%
    %         \begin{tikzpicture}[
    %             >=latex,
    %             font=\sffamily\small,
    %             layer/.style={draw, rounded corners=2pt, minimum width=2.6cm, minimum height=0.42cm, inner sep=0pt},
    %             layerbase/.style={layer, fill=blue!8, draw=blue!30},
    %             layerrl/.style={layer, fill=green!10, draw=green!50!black!30},
    %             layerpatch/.style={layer, fill=orange!18, draw=orange!65, thick},
    %             annot/.style={font=\sffamily\scriptsize, text=black!60},
    %         ]
    %             % ── Base stack ──
    %             \node[annot, font=\sffamily\footnotesize\bfseries, text=black] at (0, 3.95) {Base};
    %             \node[layerbase] (b1) at (0, 0)    {\tiny Layers 0\,--\,5};
    %             \node[layerpatch](b2) at (0, 0.60) {\tiny Layers 6\,--\,8};
    %             \node[layerbase] (b3) at (0, 1.20) {\tiny Layers 9\,--\,17};
    %             \node[layerbase] (b4) at (0, 1.80) {\tiny Layers 18\,--\,26};
    %             \node[layerbase] (b5) at (0, 2.40) {\tiny Layers 27\,--\,34};
    %             % Input
    %             \node[annot] at (0, -0.52) {Prompt $\mathbf{x}$};
    %             \draw[->, thick, blue!40] (0, -0.35) -- (b1.south);
    %             % Output
    %             \draw[->, thick, blue!40] (b5.north) -- (0, 2.75);
    %             \node[draw, rounded corners=3pt, fill=orange!8, inner sep=3pt, 
    %                   font=\sffamily\scriptsize, text=black!80] 
    %                 (out) at (0, 3.35) {``\,D'abord, calculons\,...\,''};
    %             \draw[->, thick, blue!40] (0, 2.75) -- (out.south);
    %             % Replaced annotation
    %             \node[annot, text=orange!70!black, font=\sffamily\tiny\itshape, 
    %                   anchor=west] at (1.65, 0.70) {replaced};

    %             % ── RL-GRPO stack ──
    %             \node[annot, font=\sffamily\footnotesize\bfseries, text=black] at (4.5, 3.95) {RL-GRPO};
    %             \node[layerrl] (r1) at (4.5, 0)    {\tiny Layers 0\,--\,5};
    %             \node[layerrl, fill=green!22, draw=green!50!black!50, thick] 
    %                            (r2) at (4.5, 0.60) {\tiny Layers 6\,--\,8};
    %             \node[layerrl] (r3) at (4.5, 1.20) {\tiny Layers 9\,--\,17};
    %             \node[layerrl] (r4) at (4.5, 1.80) {\tiny Layers 18\,--\,26};
    %             \node[layerrl] (r5) at (4.5, 2.40) {\tiny Layers 27\,--\,34};
    %             % Mean annotation
    %             \node[annot, align=center] at (4.5, -0.58) 
    %                 {$\bar{\mathbf{h}}^{(L)} \!=\! \frac{1}{N}\!\sum_i \mathbf{h}^{(L)}_i$
    %                  {\tiny\,at \texttt{<think>}}};

    %             % ── Patching arrow (label shifted up) ──
    %             \draw[->, thick, orange!75!black, densely dashed] 
    %                 (r2.west) -- (b2.east) 
    %                 node[midway, above=5pt, font=\sffamily\tiny, text=orange!65!black] 
    %                 {$\bar{\mathbf{h}}^{(6\text{-}8)}_{\text{RL}}$};

    %             % ── Brace ──
    %             \draw[decorate, decoration={brace, amplitude=3pt, mirror}, thick, orange!65!black] 
    %                 ([xshift=-0.25cm]b2.south west) -- ([xshift=-0.25cm]b2.north west)
    %                 node[midway, left=4pt, annot, text=orange!65!black, align=center, 
    %                      font=\sffamily\tiny] {language\\[-2pt]bottleneck};

    %             % ── Caption-like annotation at bottom ──
    %             \node[annot, text width=9cm, align=center, text=black!55] at (2.25, -1.35)
    %                 {Inject mean RL-GRPO hidden states into Base at layer $L$.\\
    %                  Measure target-language fraction of generated output.};
    %         \end{tikzpicture}%
    %         }%
    %         \caption*{Patching schematic}
    %     \end{subfigure}
    % \end{minipage}

    \caption{
    Mechanistic analysis of representation changes across training stages (Base $\to$ SFT $\to$ RL) on \underline{French} MGSM prompts.
    \textbf{(a)}~Cosine similarity between model pairs at each layer reveals a pronounced valley in layers 6--8 for both fine-tuned models relative to Base, \textbf{indicating a localized representational restructuring early in the network}. The SFT-vs-RL curve remains close to 1.0 throughout, confirming that RL preserves the geometry established by SFT.
    \textbf{(b)}~Single-layer activation patching: for each layer $L$, the mean RL hidden state at \texttt{<think>} is injected into Base, and the target-language fraction of the generated output is measured (see patching schematic). Patching layers 6--8 shifts the base model's output into French (fraction $\approx 0.8$), while all other layers produce negligible effect, \textbf{revealing a sharp causal bottleneck that coincides exactly with the drift valley in~(a)}.
    % \textbf{(c)}~Schematic of the patching procedure: mean hidden states are computed from RL-GRPO at the \texttt{<think>} token across 150 source prompts, then injected into the corresponding layer of the base model during the first generation step. Only the orange-highlighted layers causally shift the output language.
    % The results for the other languages follow similar patterns and are provided in the Appendix.
    }
    \label{fig:mechanistic-activations}
\end{figure}


\subsection{Activation Change Analysis}

We complement the weight-level view with two activation-level diagnostics, each computed from last-token hidden-states extracted at every layer. 

\textbf{Activation Drift.}
We compute the pairwise cosine similarity between hidden states of different model pairs at each layer, averaged over the 250 prompts (Figure~\ref{fig:mechanistic-activations}a). 
SFT and RL representations remain highly similar throughout the network (cosine $>0.95$ in most layers), confirming that RL preserves the representational geometry established by SFT. 
The comparison of both fine-tuned models against Base, however, reveals an interesting non-monotonic pattern: cosine similarity drops sharply in layers 6--8, forming a pronounced valley, before partially recovering in the middle layers and diverging again toward the final layers. 
This early dip is barely present in the SFT-vs-RL curve, indicating that it reflects a representational restructuring shared by both fine-tuned checkpoints relative to the pretrained model. 
The valley suggests that language-specific adaptation involves a localized transformation in the early-to-mid layers.

\textbf{Activation Patching.}
To test whether the layers identified by activation drift are \emph{causally} responsible for the language switch, we perform single-layer activation patching \citep{vig2020causalmediationanalysisinterpreting, meng2023locatingeditingfactualassociations} (Figure~\ref{fig:mechanistic-activations}b). 
For each layer $L$, we compute the mean RL hidden state at the \texttt{<think>} token over 150 held-out source prompts and inject it into the corresponding layer of the (English) base model during the first generation step, then measure the fraction of output tokens in the target language over 100 evaluation prompts.

The results reveal a causal bottleneck: patching layers 6--8 shifts the base model's output substantially toward the target language (French fraction $\approx 0.8$ at the peak), while patching any other layer, including the deep layers where weight changes are largest, produces negligible language shift (fraction $\approx 0.01$, matching clean Base). 
This mirrors the valley observed in the activation drift analysis: the layers where fine-tuned and base representations diverge the most are exactly the layers that causally control the language of generation.

These diagnostics suggest a division of labor across depth.
The early layers ($\approx$\,6--8) act as a \emph{language-routing bottleneck}: fine-tuning rewires this narrow band to steer generation into the target language.
The deeper layers, despite accumulating the largest weight updates (cf.\ Figure~\ref{fig:mechanistic-weights}), likely refine reasoning and output quality \emph{within} the language already selected by the earlier layers. 
This suggests that the early-layer bottleneck gates a global property of the output (its language), while the content-level adaptation occurs in the upper layers.

% \paragraph{Effective Dimensionality.}
% We stack the 250 last-token hidden states into a matrix at each layer, compute its SVD \citep{klema1980singular}, and report the participation ratio $\text{PR} = (\sum \sigma_i^2)^2 / \sum \sigma_i^4$ \citep{gao2017theory}, which estimates the effective number of dimensions used by the representation (Figure~\ref{fig:mechanistic-activations}b). The base model shows a pronounced collapse in the later layers, with the participation ratio dropping sharply, indicating that German representations converge to a low-dimensional subspace. SFT partially counteracts this collapse, and RL-GRPO further strengthens it, maintaining consistently higher dimensionality through the final layers. 

% \paragraph{Logit-Lens KL Divergence.}
% To measure how adaptation changes the model's internal ``predictions'' at each depth, we apply the logit-lens technique \citep{Nostalgebraist2020}: at every layer, we project the hidden state through the final layer norm and unembedding matrix, compute a softmax distribution, and measure the KL divergence from the corresponding base-model distribution (Figure~\ref{fig:mechanistic-activations}c). Notably, RL-GRPO exhibits substantially larger divergence than SFT in the final layers (layers 28--34), despite inducing smaller weight changes (cf.\ Figure~\ref{fig:mechanistic-weights}). This decoupling between weight magnitude and predictive divergence suggests that RL achieves a more efficient representational rerouting: it produces a greater departure in the model's output distribution with proportionally less parameter change, pointing to a qualitatively different optimization dynamic than supervised learning.
